Relative Upper Confidence Bound for the K-Armed Dueling Bandit Problem

This paper proposes a new method for the K-armed dueling bandit problem, a variation on the regular K-armed bandit problem that offers only relative feedback about pairs of arms. Our approach extends the Upper Confidence Bound algorithm to the relative setting by using estimates of the pairwise probabilities to select a promising arm and applying Upper Confidence Bound with the winner as a benchmark. We prove a finite-time regret bound of order O(log t). In addition, our empirical results using real data from an information retrieval application show that it greatly outperforms the state of the art.

==> lemmas.tex <==
{\bf I don't think we need to reference Bishop here: we should assume these basics are common knowledge.}

{\bf Sketch the high-level proof structure here.}

We begin with two lemmas regarding sampling from Beta posteriors, which are proven in the supplementary material.

% \begin{lemma}\label{lem:ProbBound} Given a Bernoulli random variable $X \sim \textup{Ber}(p)$ with a uniform prior (i.e. $\textup{Beta}(1,1)$) on the unknown parameter $p \in [0,1]$, and given $t$ observations from $X$, resulting in the posterior $\textup{Beta}(s,t-s)$, where $s$ is the number of successes (i.e. number of times $X$ was equal to $1$), then for any $\Delta$, we have 
% \[ P\left(\theta \notin [p-\Delta,p+\Delta] | \theta \sim \textup{Beta}(s,t-s) \right) < \frac{1}{\Delta}e^{-\frac{t}{24}} ???  \]
% \end{lemma}

\begin{mydefinition} Given $n$ pulls of a Bernoulli arm with prior $\Pi^0$ and posterior $\Pi^n$, we define the CDF of the \emph{marginalized posterior} as follows:
\[ P\left(\Pi^n > \alpha\right) := \sum_{s=0}^n p(s|n) P\left(\theta_n > \alpha|s,n\right), \]
where $\theta_n \sim \Pi^n$ is a sample from the posterior and $s$ is the number of times the arm produced a $1$.
\end{mydefinition}

\begin{lemma}\label{lem:BetaEstimate} Let $X_1, \ldots , X_n$ be a sequence of samples where $X_i \sim \textup{Ber}(p)$, $\Pi^0$ a uniform prior on $p$, and $\Pi^n$ the posterior obtained after observing the sequence of samples. Given a sample $\theta \sim \Pi^n$, we have
\[ P\left(\Pi^n > \frac{1}{2}\right) = P\left(\sum_{i=1}^n X_i + \sum_{i=1}^{n+1} Y_i
%X_1+\cdots+X_n+Y_1+\cdots+Y_{n+1} 
\geq n+1\right), \]
where $Y_i \sim \textup{Ber}(\frac{1}{2})$ and by $P\left(\theta > \frac{1}{2} | n \right)$ we mean the probability of the event $\theta > \frac{1}{2}$ given that $n$ samples from $X_i \sim \textup{Ber}(p)$ have been observed. From this we can conclude
\begin{align*}
P\left(\sum_{i=1}^n X_i + Y_i \geq n+1 \right) \leq P\left(\theta > \frac{1}{2} \bigg| n \right) \leq P\left(\sum_{i=1}^{n+1} X_i + Y_i \geq n+1\right).
\end{align*}
\end{lemma}

\begin{lemma}\label{lem:BetaTailShrinkage} Let $X_1, \ldots , X_n$ be a sequence of samples where $X_i \sim \textup{Ber}(p)$, $\Pi^0$ a uniform prior on $p$, with $p < \frac{1}{2}$, and $\Pi^n$ the posterior obtained after observing the sequence of samples. Then, we have for each $n$
\[ P\left(\Pi^n > \frac{1}{2}\right) > P\left(\Pi^{n+1} > \frac{1}{2}\right) \]
\end{lemma}

\begin{lemma}\label{lem:BinomialEstimate} Given random variables $X_1, \ldots, X_n$ where $X_i \sim \textup{Ber}(p)$ and $p < \frac{1}{2}$, and $Y_1, \ldots Y_n$ where $Y_i \sim \textup{Ber}(\frac{1}{2})$, we have the following pair of bounds:
\begin{align}
\left(\frac{p}{2}\right)^n \leq P\left(\sum_{i=1}^n X_i+Y_i \geq n+1\right) < P\left(\sum_{i=1}^n X_i+Y_i\geq n\right) \leq e^{-\frac{n\Delta^2}{2}}, \label{eqn:LUB}
\end{align}
where $\Delta := \frac{1}{2}-p$.
\end{lemma}

\begin{remark}
Putting together the bounds in Lemmas \ref{lem:BetaEstimate} and \ref{lem:BinomialEstimate}, we have the following envelope for $n \geq 1$:
\[  \left(\frac{p}{2}\right)^n \leq P\left(\theta > \frac{1}{2} \bigg| n \right) \leq e^{-\frac{(n+1)\Delta^2}{2}} \]
\end{remark}


%%%% NOTE from Masrour: I'm commenting this out.
% \begin{lemma} 
% If on the $t$-th iteration of RTS, the best arm wins the round-robin tournament, i.e., $c=1$ (line 13), then there exists an integer $L$ such that
% \[  P(r_t > 0) \leq \frac{L}{n}, \]
% where $r_t$ is the absolute regret incurred by the regular TS algorithm run in the second step (lines 15--20) of that iteration.
% \end{lemma}
% 
% \begin{proof}
% Let  $\mathcal E_t$ be the event that on the $t$-th iteration of RTS, for every $\theta_{cj}$ sampled on line 18, $\theta_{cj} < \frac{1}{2}$.  Note that, if $c=1$, then $r_t > 0 \Leftrightarrow \overline{\mathcal E}_t$, where $\overline{\mathcal E}_t$ is the complement of $\mathcal E_t$.
% {\bf From here, cut Prop 4 and Remark 5, and continue the proof of Lem 3 using the proof of Remark 5, but replacing $\mathcal E_n$ with $\mathcal E_t$}.
% \end{proof}
%%% END NOTE

%We need the following definition in what follows:
%\begin{mydefinition}\label{def:E} Given $\theta_{ij}$ as in Algorithm \ref{alg:RTS}, we denote by $\mathcal E_c$ the event that $\theta_{ij} < \frac{1}{2}$ whenever $i = c$ and  $\theta_{ij} > \frac{1}{2}$ whenever $j = c$. Note that the algorithm accumulates no regret exactly when $\mathcal E_c$ happens twice in a row, where $c$ is the true champion.
%\end{mydefinition}
%
%
%\begin{proposition}\label{prop:AbsBandits} Consider the following regular bandit problem with $K$ arms, with $X_1, \ldots, X_K$ the corresponding random variables: we will assume that $X_1 = \frac{1}{2}$ almost surely, and that for $i > 1$ we have $X_i \sim \textup{Ber}(p_i)$, satisfying $p_i < \frac{1}{2}$ for $i > 1$. Then, there exists an integer $L$ such that we have the following bound:
%\[  P(r_n > 0) \leq \frac{L}{n}, \]
%where $n$ denotes the number of iterations of the algorithm.
%\end{proposition}
%
%\begin{remark}\label{rmk:AbsBandits} Note that the setup of this proposition and the part II of Algorithm \ref{alg:RTS} are identical up to reordering of the indices so that the $c^{th}$ arm is mapped to the first one, and in fact the event $\{r_t > 0\}$ corresponds precisely to the complement of the event $\mathcal E$, defined in Definition \ref{def:E}, so this proposition gives us a lower bound on the probability of $\mathcal E$. We will denote the compliment of $\mathcal E$ by $\overline{\mathcal E}$.
%\end{remark}

